Asymmetric Image Retrieval with Cross Model Compatible Ensembles

The asymmetrical retrieval setting is a well suited solution for resource constrained applications such as face recognition and image retrieval. In this setting, a large model is used for indexing the gallery while a lightweight model is used for querying. The key principle in such systems is ensuring that both models share the same embedding space. Most methods in this domain are based on knowledge distillation. While useful, they suffer from several drawbacks: they are upper-bounded by the performance of the single best model found and cannot be extended to use an ensemble of models in a straightforward manner. In this paper we present an approach that does not rely on knowledge distillation, rather it utilizes embedding transformation models. This allows the use of N independently trained and diverse gallery models (e.g., trained on different datasets or having a different architecture) and a single query model. As a result, we improve the overall accuracy beyond that of any single model while maintaining a low computational budget for querying. Additionally, we propose a gallery image rejection method that utilizes the diversity between multiple transformed embeddings to estimate the uncertainty of gallery images.

==> comparison_to_alternatives.tex <==
\subsection{Comparison to other ensemble alternatives}
To further validate our ensemble design choices we compare our approach to alternative ensemble architectures.
We present alternative approaches to our proposed method of using independently trained transformation models, one for each gallery model, and averaging the transformed embeddings.
Instead of the above, we learn a single combined transformation model that takes embeddings from all gallery models as inputs, and outputs a transformed embedding in the query model's embedding space.
Since creating a single combined transformation model is not straightforward, we propose multiple variants:
\begin{enumerate}
    \item \textbf{End-to-end averaging:} We train a transformation model from each gallery model to the query embedding space simultaneously.
    The difference between this variant to our method is that instead of training each transformation model independently, we train all transformation models together and perform the averaging during training.
    \item \textbf{Weighted end-to-end averaging:}  In a similar manner, we jointly train all transformation models except that we use weighted averaging instead of simple averaging.
    %The weights are each transformation model also outputs 
    Each transformation model outputs a single scalar value, in addition to the embedding output, that is used for weighting in averaging operation.
    \item \textbf{Concatenation:} All gallery embeddings are first concatenated and
    inserted into a linear layer reducing the dimensions.
    The output of the linear layer is then transformed by a single transformation model to the embedding space of the query model.
\end{enumerate}
In this experiment, for all variants, and for our method, we used the same five pre-trained ResNet18 models. One for the query model, and four for the gallery models.

\input{figures/table_alternative_ensemble}

Table~\ref{tab:table_alternative_ensemble} presents the comparison between our ensemble approach and the combined transformation variants.
The results indicate that our approach performers considerably better then the other variants.
Furthermore, this implies that explicitly optimizing the ensemble performs worse than averaging independently trained models.
A similar phenomenon is also observed and discussed by Lee~\etal~\cite{lee2015m}.
% An additional and meaningful advantage of our approach takes effect in test time.
% Each time the embedding model is updated, we need to train new transformers from all the existing gallery embeddings to the new embedding model.
% Considering we have $N$ gallery embedding models, training $N$ different transformers effectively takes much less time then training a single transformer with a very large input space ($N$ times the size of each embedding).

==> figures/fig_ensemble_types.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.38\textwidth}
         \centering
         %\raisebox{1.9 em}{\includegraphics[width=0.9\textwidth]{figures/ensemble_types/DT}}
         %\raisebox{1.9 em}{\includegraphics[width=0.9\textwidth]{images/a.pdf}}
         \includegraphics[width=0.9\textwidth]{images/diversity/dt.pdf}
         \vspace{13pt}
         \caption{D-T.}
         \label{fig:ensemble_type_DT}
     \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         %\includegraphics[width=0.9\textwidth]{figures/ensemble_types/DTG}
         %\includegraphics[width=0.9\textwidth]{images/b.pdf}
         \includegraphics[width=0.9\textwidth]{images/diversity/dtg.pdf}
         \caption{D-TG.}
         \label{fig:ensemble_type_DTG}
     \end{subfigure}
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         %\includegraphics[width=0.9\textwidth]{figures/ensemble_types/DTGA}
         %\includegraphics[width=0.9\textwidth]{images/c.pdf}
         \includegraphics[width=0.9\textwidth]{images/diversity/dtga.pdf}
         \caption{D-TGA.}
         \label{fig:ensemble_type_DTGA}
     \end{subfigure}
    \caption{\textbf{Ensemble diversity levels.} 
    %$N$ Transformation models $\{T_i\}_{i=1}^N$ are used for the ensemble.
    D-T: Multiple transformation models are learned to map the embedding vectors of a single gallery model to the space of the query model.
    % D-TG: A single transformation model is learned for each different gallery model, where each gallery model has the same architecture, \eg, ResNet100.
    D-TG: For each gallery model a different transformation model is learned and all gallery models share the \textbf{same} architecture, \eg, ResNet18.
    D-RGA: For each gallery model a different transformation model is learned and gallery models may use \textbf{different} architectures, \eg, ResNet100, ResNet18 and MBF.
    %D-RGA: A single transformation is learned for a different, varying-architecture, gallery model (colors represents a different $\phi_g$ architectures), \eg, ResNet100, ResNet18 and MBF.
    }
    \label{fig:ensemble_type_plot}
\end{figure*}

==> figures/fig_mix_of_models.tex <==
\begin{figure}
    \includegraphics[width=\textwidth]{images/mix_of_models_concept.png}
    \caption{TODO.}
    \label{fig:mix_of_models}
\end{figure}

==> figures/fig_overview.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.92\textwidth]{images/overveiw.pdf}
    \caption{\textbf{System Overview.}
    Visual search system have two modes: indexing of gallery images and querying test images.
    Leveraging the fact that indexing is performed offline, we propose to use multiple gallery models, $\phi^i_g$.
    %at this stage. 
    Since the gallery models' embedding spaces are not compatible, transformation models $T_i$ are used to map their embeddings to that of the query model, $\phi_q$.
    Thus, we allow higher accuracy without sacrificing efficiency under the cross model compatibility (CMC) requirement.
    } 
    \label{fig:overview}
\end{figure*}

==> figures/fig_proposed_approach.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         %\includegraphics[width=0.9\textwidth]{figures/proposed_approach/unified}
         \includegraphics[height=110pt]{images/unified.pdf}
         \caption{Unified Space}
         \label{fig:proposed_unified}
     \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         %\includegraphics[width=0.9\textwidth]{figures/proposed_approach/m2m}
         \includegraphics[height=110pt]{images/m2m.pdf}
         \caption{Model-to-model}
         \label{fig:proposed_m2m}
     \end{subfigure}
        \begin{subfigure}[b]{0.38\textwidth}
         \centering
         %\raisebox{0.27 em}{\includegraphics[width=0.99\textwidth]{figures/proposed_approach/ensemble}}
         \includegraphics[height=110pt]{images/ensemble.pdf}
         \caption{Ensemble}
         \label{fig:proposed_ensemble}
     \end{subfigure}
    \caption{\textbf{Ensemble of transformation models.} 
    (a) In the unified space approach of Wang~\etal~\cite{wang2020unified}, both the gallery's and the query's models' ($\phi_g$, $\phi_q$) embedding spaces are transformed to a unified space.
    (b) The model-to-model (m2m) approach directly transforms $\phi_g$'s embeddings to $\phi_q$'s embedding space.
    (c) An ensembles of m2m transformation models %is created by averaging the results of multiple transformation models, which
    transform embeddings from $N$ different gallery models, $\{\phi_g^i\}_{i=1}^N$, to the same embedding space of $\phi_q$.
    }
    \label{fig:proposed_approach}
\end{figure*}

==> figures/fig_table_comp.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.54\textwidth}
        \centering
        \small{
        \begin{tabular}{l|cc}
            \toprule
            {} & 1:N search & 1:1 verification \\
            {} & @FAR=1\% & @FAR=0.01\% \\
            \midrule
            No-CMC: $\phi_g=\phi_q$ & 20.157\tiny{$\pm 0.50$} & 11.936\tiny{$\pm 0.27$}\\
            \midrule
            Unified~\cite{wang2020unified} & 19.353\tiny{$\pm 0.32$}  & 11.561\tiny{$\pm 0.14$} \\
            Model-to-model &  19.524\tiny{$\pm0.29$}  & 11.632\tiny{$\pm0.12$} \\
            \midrule
            Ensemble of 2 & 18.583 & 10.932 \\
            Ensemble of 4 & 18.068 & 10.861 \\
            Ensemble of 9 & \textbf{17.759} & \textbf{10.656} \\
            \bottomrule
        \end{tabular}
        }
        \caption{1:N search and 1:1 verification (FRR).}
        \label{table:basline_comp}
    \end{subfigure}
    \begin{subfigure}[b]{0.44\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth]{images/res18_rec.pdf}
         \caption{1:N search FRR vs. ensemble size.}
         \label{fig:basline_comp}
    \end{subfigure}
    \caption{\textbf{Comparison to baselines.}
    Table~(a) shows 1:N search and 1:1 verification FRR (in percentage) at fixed FAR values for our method (with ensemble sizes: 2, 4 and 9) and the baselines our methods builds upon.
    No-CMC, $\phi_g=\phi_q$, was evaluated on ten ResNet18 models.
    Unified and Model-to-model were evaluated on ten different $\phi_g$ ResNet18 models and the same $\phi_q$.
    The baseline FRRs are shown as mean and std values of ten evaluations.
    Fig.~(b) shows 1:N search for different ensemble sizes.
    Since the baselines use only one gallery model they are visualized as lines.
    Note that ensemble of size one does not coincide with the Model-to-model line because the Model-to-model line represents the average of ten evaluations.   
    %with error bands in the plot (each baseline was trained ten times).  
    % All models are using the ResNet18 architecture.
    }
    %Evaluation results on the recognition and verification tasks. The percentage in the columns are FRR at fixed FAR values (e.g., 1\% means FRR results when FAR is fixed to 1\%). We compared our model2model approach to the baselines, and demonstrate how different ensemble size.}
    \label{fig:basline comp}
\end{figure*}

==> figures/fig_uncertenty_images.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.33\textwidth}
         \centering
         \footnotesize
         \setlength{\tabcolsep}{1pt}
         \begin{tabular}{ccc}
% low_443172.jpg, var: 0.181
% low_441912.jpg, var: 0.196
% low_4559.jpg, var: 0.199
% low_2089.jpg, var: 0.200
% low_30830.jpg, var: 0.202
% low_441641.jpg, var: 0.204
% low_441374.jpg, var: 0.207
% low_2449.jpg, var: 0.207
% low_1620.jpg, var: 0.209
% low_4722.jpg, var: 0.213
% low_101213.jpg, var: 0.214
% low_441563.jpg, var: 0.214
% low_441262.jpg, var: 0.215
% low_444848.jpg, var: 0.216
% low_115259.jpg, var: 0.216
            0.199 & 0.200 &0.202\\
              %\includegraphics[width=0.3\textwidth]{images/uncertinty/low_443172.jpg} &
              %\includegraphics[width=0.3\textwidth]{images/uncertinty/low_441912.jpg} &
              \includegraphics[width=0.3\textwidth]{images/uncertainty/low_4559.jpg} &
              \includegraphics[width=0.3\textwidth]{images/uncertainty/low_2089.jpg} &
              \includegraphics[width=0.3\textwidth]{images/uncertainty/low_30830.jpg} \\
            0.204 & 0.207 & 0.207 \\
              \includegraphics[width=0.3\textwidth]{images/uncertainty/low_441641.jpg} &
              \includegraphics[width=0.3\textwidth]{images/uncertainty/low_441374.jpg} &
              \includegraphics[width=0.3\textwidth]{images/uncertainty/low_2449.jpg} \\
            % 0.209 & 0.213 & 0.214 \\
            %   \includegraphics[width=0.3\textwidth]{images/uncertainty/low_1620.jpg} & 
            %   \includegraphics[width=0.3\textwidth]{images/uncertainty/low_4722.jpg} &
            %   \includegraphics[width=0.3\textwidth]{images/uncertainty/low_101213.jpg} \\
            
            
            % 0.214 & 0.215 & 0.216 \\
            %   \includegraphics[width=0.3\textwidth]{images/uncertinty/low_441563.jpg} &
            %   \includegraphics[width=0.3\textwidth]{images/uncertinty/low_441262.jpg} &
            %   \includegraphics[width=0.3\textwidth]{images/uncertinty/low_444848.jpg} \\
         \end{tabular}
         \caption{Low level variance.}
         \label{fig:low_variance}
     \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
         \centering
         \footnotesize
         \setlength{\tabcolsep}{1pt}
         \begin{tabular}{ccc}
%mid_2883.jpg, var: 0.342
%mid_448861.jpg, var: 0.342
%mid_74503.jpg, var: 0.342
%mid_440525.jpg, var: 0.342
%mid_562.jpg, var: 0.342
%mid_448720.jpg, var: 0.342
%mid_442082.png, var: 0.343
%mid_442951.jpg, var: 0.343
%id_101952.jpg, var: 0.343
%mid_111561.jpg, var: 0.343
%mid_440358.jpg, var: 0.343
%mid_2638.jpg, var: 0.343
%mid_1798.jpg, var: 0.344
            0.342 & 0.342 & 0.342 \\
              \includegraphics[width=0.3\textwidth]{images/uncertainty/mid_2883.jpg} &
              \includegraphics[width=0.3\textwidth]{images/uncertainty/mid_448861.jpg} &
              \includegraphics[width=0.3\textwidth]{images/uncertainty/mid_74503.jpg} \\
            0.342 & 0.342 & 0.342 \\
              \includegraphics[width=0.3\textwidth]{images/uncertainty/mid_440525.jpg} &
              \includegraphics[width=0.3\textwidth]{images/uncertainty/mid_562.jpg} &
              \includegraphics[width=0.3\textwidth]{images/uncertainty/mid_448720.jpg} \\
            % 0.343 & 0.343 & 0.343 \\
            %   \includegraphics[width=0.3\textwidth]{images/uncertainty/mid_442082.png} &
            %   \includegraphics[width=0.3\textwidth]{images/uncertainty/mid_442951.jpg} &
            %   \includegraphics[width=0.3\textwidth]{images/uncertainty/mid_101952.jpg} \\
            
            
            
            % 0.343 & 0.343 & 0.343 \\
            %   \includegraphics[width=0.3\textwidth]{images/uncertinty/mid_111561.jpg} &
            %   \includegraphics[width=0.3\textwidth]{images/uncertinty/mid_440358.jpg} &
            %   \includegraphics[width=0.3\textwidth]{images/uncertinty/mid_2638.jpg} \\
         \end{tabular}
         \caption{Medium level variance.}
         \label{fig:mid_variance}
     \end{subfigure}
        \begin{subfigure}{0.33\textwidth}
         \centering
         \footnotesize
         \setlength{\tabcolsep}{1pt}
         \begin{tabular}{ccc}
% high_2899.jpg, var: 0.430
% high_447599.jpg, var: 0.436
% high_449009.jpg, var: 0.441
% high_108674.jpg, var: 0.456
% high_1718.jpg, var: 0.471
% high_109637.jpg, var: 0.481
% high_447382.jpg, var: 0.483
% high_447310.jpg, var: 0.483
% high_444830.jpg, var: 0.491
% high_447740.jpg, var: 0.496
% high_446773.jpg, var: 0.508
% high_442264.jpg, var: 0.511
% high_442672.png, var: 0.524
% high_447699.jpg, var: 0.547
% high_112173.jpg, var: 0.576
            %\vspace{-1.pt}
            0.576 & 0.547 & 0.524 \\
              \includegraphics[width=0.3\textwidth]{images/uncertainty/high_112173.jpg} &
              \includegraphics[width=0.3\textwidth]{images/uncertainty/high_447699.jpg} &
              \includegraphics[width=0.3\textwidth]{images/uncertainty/high_442672.png} \\
            0.511 & 0.508 & 0.496 \\
              \includegraphics[width=0.3\textwidth]{images/uncertainty/high_442264.jpg} &
              \includegraphics[width=0.3\textwidth]{images/uncertainty/high_446773.jpg} &
              \includegraphics[width=0.3\textwidth]{images/uncertainty/high_447740.jpg} \\
            % 0.491 & 0.483 & 0.483 \\
            %   \includegraphics[width=0.3\textwidth]{images/uncertainty/high_444830.jpg} &
            %   \includegraphics[width=0.3\textwidth]{images/uncertainty/high_447310.jpg} &
            %   \includegraphics[width=0.3\textwidth]{images/uncertainty/high_447382.jpg} \\
            
            
            
            % 0.481 & 0.471 & 0.456 \\
            %   \includegraphics[width=0.3\textwidth]{images/uncertinty/high_109637.jpg} &
            %   \includegraphics[width=0.3\textwidth]{images/uncertinty/high_1718.jpg} &
            %   \includegraphics[width=0.3\textwidth]{images/uncertinty/high_108674.jpg} \\
         \end{tabular}
         %\includegraphics[height=0.3\textwidth]{images/unified.pdf}
         \caption{High level variance.}
         \label{fig:high_variance}
     \end{subfigure}
    \caption{%\textbf{Gallery images with different levels of variance.}
    Examples of gallery images with (a) low, (b) medium and (c) high variance values.
    The numbers above the images shows the corresponding variance value.% of the gallery template and the image is randomly sampled out of the template images
    }
    \vskip -0.07in
    \label{fig:uncertenty_images}
\end{figure*}

% high_449009.jpg, var: 0.530
% high_441932.jpg, var: 0.533
% high_441346.jpg, var: 0.538
% high_108674.jpg, var: 0.547
% high_1718.jpg, var: 0.548
% high_447382.jpg, var: 0.562
% high_444830.jpg, var: 0.576
% high_442264.jpg, var: 0.577
% high_109637.jpg, var: 0.585
% high_442672.png, var: 0.595
% high_447740.jpg, var: 0.599
% high_446773.jpg, var: 0.605
% high_447310.jpg, var: 0.610
% high_447699.jpg, var: 0.613
% high_112173.jpg, var: 0.681
% mid_4151.jpg, var: 0.339
% mid_107758.jpg, var: 0.339
% mid_216.jpg, var: 0.339
% mid_101140.jpg, var: 0.339
% mid_441530.jpg, var: 0.339
% mid_4634.jpg, var: 0.339
% mid_445128.jpg, var: 0.339
% mid_109024.jpg, var: 0.339
% mid_38991.jpg, var: 0.339
% mid_102277.jpg, var: 0.339
% mid_440676.jpg, var: 0.339
% mid_2513.jpg, var: 0.339
% mid_101124.jpg, var: 0.339
% mid_441315.jpg, var: 0.339
% mid_440532.jpg, var: 0.339
% low_1269.jpg, var: 0.246
% low_445794.jpg, var: 0.250
% low_78944.jpg, var: 0.253
% low_44754.jpg, var: 0.258
% low_445236.jpg, var: 0.258
% low_51762.jpg, var: 0.259
% low_2289.jpg, var: 0.259
% low_446545.jpg, var: 0.260
% low_451545.jpg, var: 0.264
% low_111887.jpg, var: 0.267
% low_446166.jpg, var: 0.269
% low_445980.jpg, var: 0.271
% low_449792.jpg, var: 0.271
% low_440639.jpg, var: 0.272
% low_441374.jpg, var: 0.272


==> figures/simulation.tex <==
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.44\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth]{images/sim_rec.pdf}
         \caption{1:N search}
         \label{fig:sim_rec}
     \end{subfigure}
     \begin{subfigure}[b]{0.44\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth]{images/sim_var.pdf}
         \caption{1:1 verification}
         \label{fig:sim_rec}
     \end{subfigure}
        \caption{Simulation} 
        \label{fig:simulation}
\end{figure}
